Model Predictive Control Based Trajectory Generation for Autonomous Vehicles - An Architectural Approach

Research in the field of automated driving has created promising results in the last years. Some research groups have shown perception systems which are able to capture even complicated urban scenarios in great detail. Yet, what is often missing are general-purpose path- or trajectory planners which are not designed for a specific purpose. In this paper we look at path- and trajectory planning from an architectural point of view and show how model predictive frameworks can contribute to generalized path- and trajectory generation approaches for generating safe trajectories even in cases of system failures.

==> figures/constraintSteps.tex <==
\begin{tikzpicture}
\input{../constraintsSteps.TpX}
\end{tikzpicture}

==> figures/tikz/shapes.tex <==
%
% declare a new shape for the service interface
\makeatletter
\pgfdeclareshape{openinterface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
}
\pgfdeclareshape{interface}
{
  \inheritsavedanchors[from=circle] % this is nearly a circle
  \inheritanchorborder[from=circle]
  \inheritanchor[from=circle]{north}
  \inheritanchor[from=circle]{north west}
  \inheritanchor[from=circle]{north east}
  \inheritanchor[from=circle]{center}
  \inheritanchor[from=circle]{west}
  \inheritanchor[from=circle]{east}
  \inheritanchor[from=circle]{mid}
  \inheritanchor[from=circle]{mid west}
  \inheritanchor[from=circle]{mid east}
  \inheritanchor[from=circle]{base}
  \inheritanchor[from=circle]{base west}
  \inheritanchor[from=circle]{base east}
  \inheritanchor[from=circle]{south}
  \inheritanchor[from=circle]{south west}
  \inheritanchor[from=circle]{south east}
  \backgroundpath{
    \centerpoint%
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
	 \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{+1pt}{.95\pgfutil@tempdima}}}
    \pgfpatharc{80}{280}{\pgfutil@tempdima}
  }
  \foregroundpath{
	 \centerpoint
    \pgf@xc=\pgf@x%                 \pgf@xc = x value of centerpoint
    \pgf@yc=\pgf@y%                 \pgf@yc = y value of centerpoint
    \pgfutil@tempdima=\radius%      \pgfutil@tempdima = radius
    \pgfutil@tempdimb=\radius%      \pgfutil@tempdima = radius
	 \advance\pgfutil@tempdima by-.25\pgfutil@tempdima%
	 \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+.25\pgfutil@tempdimb}{0pt}}}{\pgfutil@tempdima}
	 \pgfusepath{fill}
  }
}
% UML component
\pgfdeclareshape{umlcomponent}
{
  \inheritsavedanchors[from=rectangle] % this is nearly a rectangle
  \inheritanchorborder[from=rectangle]
  \inheritanchor[from=rectangle]{north}
  \inheritanchor[from=rectangle]{north west}
  \inheritanchor[from=rectangle]{north east}
  \inheritanchor[from=rectangle]{center}
  \inheritanchor[from=rectangle]{west}
  \inheritanchor[from=rectangle]{east}
  \inheritanchor[from=rectangle]{mid}
  \inheritanchor[from=rectangle]{mid west}
  \inheritanchor[from=rectangle]{mid east}
  \inheritanchor[from=rectangle]{base}
  \inheritanchor[from=rectangle]{base west}
  \inheritanchor[from=rectangle]{base east}
  \inheritanchor[from=rectangle]{south}
  \inheritanchor[from=rectangle]{south west}
  \inheritanchor[from=rectangle]{south east}
  \backgroundpath{
	  \newdimen\pgf@xd\newdimen\pgf@yd
	  \newdimen\pgf@xe\newdimen\pgf@ye
	  \newdimen\pgf@xf\newdimen\pgf@yf
		% store lower right in xa/ya and upper right in xb/yb
		\southwest \pgf@xa=\pgf@x \pgf@ya=\pgf@y
		\northeast \pgf@xb=\pgf@x \pgf@yb=\pgf@y
		% compute west point as well as vertical distance and height of decoration
		\pgf@xc=\pgf@xa \pgf@yc=.5\pgf@yb \advance\pgf@yc by .5\pgf@ya
		\pgf@yd=.3\pgf@yb
		\pgf@ye=.2\pgf@yb
%		% compute position of second decoration in xe/ye and xf/yf
%		\pgf@xe=\pgf@xa \pgf@ye=.1\pgf@y
%		\pgf@xf=\pgf@xa \pgf@yf=.2\pgf@ya
		% draw main shape
		\pgfpathmoveto{\pgfpoint{\pgf@xa}{\pgf@ya}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc-\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xa}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@yb}}
		\pgfpathlineto{\pgfpoint{\pgf@xb}{\pgf@ya}}
		\pgfpathclose
		% draw internal lines
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc-\pgf@yd-\pgf@ye}}
		\pgfpathmoveto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd+\pgf@ye}}
		\pgfpathlineto{\pgfpoint{\pgf@xc+\pgf@ye}{\pgf@yc+\pgf@yd}}
		\pgfpathlineto{\pgfpoint{\pgf@xc}{\pgf@yc+\pgf@yd}}
  }
}

% arrows
\pgfarrowsdeclare{srvarrow}{srvarrow}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.4\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.5\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{white}
  \pgfusepathqfill
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.8\pgfutil@tempdima}{0.94\pgfutil@tempdima}}}%
  \pgfpatharc{110}{-110}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke
  \pgftransformshift{\pgfqpoint{-0.5\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.55\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill
}

\pgfarrowsdeclare{srvrequired}{srvrequired}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgftransformshift{\pgfqpoint{0.35\pgfutil@tempdima}{0pt}}%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{1.3\pgfutil@tempdima}{0.95\pgfutil@tempdima}}}%
  \pgfpatharc{80}{280}{\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqstroke 
}

\pgfarrowsdeclare{srvprovided}{srvprovided}{%
  \pgfutil@tempdima=4pt\relax
  \advance\pgfutil@tempdima-\pgflinewidth
  \pgfarrowsleftextend{+-\pgfutil@tempdima}%
  \pgfarrowsrightextend{+1.5\pgflinewidth}%
}{%
  \pgfpathmoveto{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfqpoint{-0.4\pgfutil@tempdima}{.98\pgfutil@tempdima}}}%
  \pgfcircle{\pgfpointadd{\pgfqpoint{\pgf@xc}{\pgf@yc}}{\pgfpoint{+0.2\pgfutil@tempdimb}{0pt}}}{0.75\pgfutil@tempdima}
  \pgfsetfillcolor{.}
  \pgfusepathqfill 
}
\makeatother

